ACER: Automatic Language Model Context Extension via Retrieval

Long-context modeling is one of the critical capabilities of language AI for digesting and reasoning over complex information pieces. In practice, long-context capabilities are typically built into a pre-trained language model~(LM) through a carefully designed context extension stage, with the goal of producing generalist long-context capabilities. In our preliminary experiments, however, we discovered that the current open-weight generalist long-context models are still lacking in practical long-context processing tasks. While this means perfectly effective long-context modeling demands task-specific data, the cost can be prohibitive. In this paper, we draw inspiration from how humans process a large body of information: a lossy \textbf{retrieval} stage ranks a large set of documents while the reader ends up reading deeply only the top candidates. We build an \textbf{automatic} data synthesis pipeline that mimics this process using short-context LMs. The short-context LMs are further tuned using these self-generated data to obtain task-specific long-context capabilities. Similar to how pre-training learns from imperfect data, we hypothesize and further demonstrate that the short-context model can bootstrap over the synthetic data, outperforming not only long-context generalist models but also the retrieval and read pipeline used to synthesize the training data in real-world tasks such as long-context retrieval augmented generation.

==> prompts/generator.tex <==
\begin{figure}[h!]
\centering
\begin{tcolorbox}[
  enhanced,
  title=Generator Prompt,
  attach boxed title to top center={yshift=-2mm,yshifttext=-1mm},
  colback=gray!15,
  colframe=gray!75!black,
  colbacktitle=gray!40,
  coltitle=black,
  fonttitle=\bfseries,
  boxed title style={size=small,colframe=gray!50!black},
  boxrule=0.4pt,
  arc=5pt,
  outer arc=5pt,
  left=5pt, % Reduced padding
  right=5pt, % Reduced padding
  top=5pt, % Reduced padding
  bottom=5pt % Reduced padding
]
Answer the following question by reading the given passages.
\bigskip

Question: \hl{\{question\}}
\bigskip

Passages:\\
\hl{\{passages\}}
\bigskip
\bigskip

Think carefully and start your answer by first extracting a few pieces of related information from the passages.\\
Then identify the most useful piece of information and use it to answer the question.\\
On the last line, end your response with a complete full sentence answer of the following format: Answer: $<$complete answer$>$\\
Answer ``No answer was found'' if you cannot find the answer in the given passages.
\end{tcolorbox}
\caption{Prompts given to the LM to produce the final CoT answer.}
\label{fig:prompt-reader}
\end{figure}

==> prompts/ranker.tex <==
\begin{figure}[htbp]
\centering
\begin{tcolorbox}[
  enhanced,
  title=Ranker Prompt,
  attach boxed title to top center={yshift=-3mm,yshifttext=-1mm},
  colback=gray!15,
  colframe=gray!75!black,
  colbacktitle=gray!40,
  coltitle=black,
  fonttitle=\bfseries,
  boxed title style={size=small,colframe=gray!50!black},
  boxrule=0.5pt,
  arc=7pt,
  outer arc=7pt,
  left=10pt,
  right=10pt,
  top=10pt,
  bottom=10pt
]
Let's think step by step: decide if the given question can be answered by the given passage.
\bigskip

Choose from the following options:\\
a) The passage provides the exact answer to the given question.\\
b) The passage provides a partial answer to the question.\\
c) The passage provides an answer to a similar but different question.\\
d) The passage is only tangentially related to the question.\\
e) The passage is not related to the question.\\
\bigskip

The last line of your answer should be:
Answer: [a)/b)/c)/d)/e)].
\bigskip

Question:
\hl{\{question\}}
\bigskip

Passage:
\hl{\{passages\}}

\end{tcolorbox}
\caption{Prompts given to the LM to produce relevance judgement.}
\label{fig:prompt-ranker}
\end{figure}

==> tables/main.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{p{6cm}ccc}
        \toprule
        \multirow{2}{*}{\textbf{Model}} & \textbf{NQ} & \textbf{TQA} & \textbf{NarrativeQA} \\
        & (EM) & (EM) & (F1) \\
        \midrule
        \textit{Supervised Open Data}\\
        Together-Llama-2-7B-32K-Instruct & 0.172 & 0.299 & 0.013 \\
        Llama-3-8B-ProLong-512k-Instruct & 0.260 & 0.457 & 0.150\\
        
        \midrule
        \textit{Supervised Closed Data}\\
        Llama3-8B-Instruct (Truncation) & 0.388 & 0.567 & 0.076\\
        Llama3-8B-Instruct (RAG) & 0.408 & 0.611 & 0.161 \\
        Llama3.1-8B-Instruct & 0.312 & 0.518 & \textbf{0.217}\\
        Mistral-Nemo-Instruct-2407$^\text{12B}$ & 0.365 & 0.534 & 0.072\\
        \midrule
        \textit{Self-Supervised}\\
        \ours (ours) & \textbf{0.446} & \textbf{0.648} & 0.189\\
        \bottomrule
    \end{tabular}
    \caption{Performance comparison of \ours and baselines on Natural Question (NQ), TriviaQA (TQA), and NarrativeQA. The best performance on each dataset is boldfaced.}
    \label{tab:main-results}
\end{table}

==> tables/table-base-retriever.tex <==
\begin{table}[h]
\centering
\begin{tabular}{clcc}
\toprule
\multirow{2}{*}{\textbf{Retriever}} & \multirow{2}{*}{\textbf{Model}} & \textbf{NQ} & \textbf{TQA}  \\
&    & (EM) & (EM) \\
\midrule
\multirow{4}{*}{BM25}
& Llama3 (Truncation) & 0.260 &0.542 \\
& Llama3 (RAG) & 0.354 & 0.576  \\
& Llama3.1  & 0.305 & 0.507 \\
& \ours  & \textbf{0.383} & \textbf{0.632} \\
\midrule
\multirow{4}{*}{Dense}
& Llama3 (Truncation) & 0.388 & 0.567 \\
& Llama3 (RAG) & 0.408 & 0.611 \\
& Llama3.1 & 0.312 & 0.518 \\
& \ours & \textbf{0.446} & \textbf{0.648} \\
\bottomrule
\end{tabular}
\caption{Performance of \ours and baselines with different base retrievers.}
\label{tab:analysis-retrieverf}
\end{table}
% \begin{table}[h]
% \centering
% \begin{tabular}{lccc}
% \toprule
% \textbf{Model} & Retriever & \textbf{NQ} & \textbf{TQA}  \\
% &    & (EM) & (EM) \\
% \midrule
% Llama3 (Truncation) & BM25 & 0.260 &0.542 \\
% Llama3 (RAG) & BM25 & 0.354 & 0.576  \\
% Llama3.1 & BM25 & 0.305 & 0.507 \\
% \ours & BM25 & 0.383 & 0.632 \\
% \midrule
% Llama3 (Truncation) & Dense & 0.388 & 0.567 \\
% Llama3 (RAG) & Dense & 0.408 & 0.611 \\
% Llama3.1 & Dense & 0.312 & 0.518 \\
% \ours & Dense & 0.446 & 0.648 \\
% \bottomrule
% \end{tabular}
% \caption{Main Results.}
% \label{tab:analysis-retrieverf}
% \end{table}
